FASTER: Fast Adjoint Stochastic Transport for Endpoint Refinement in Reward-Guided Image Editing

Reward-guided image editing at test time seeks to improve a specified reward while preserving source content and visual plausibility. Many existing approaches optimize candidates through pretrained generation processes, making repeated adjustment depend on costly large-model execution and, in some cases, backbone backpropagation. We develop a theoretical framework that jointly accounts for reward, source preservation, and pretrained-prior preferences, allowing the desired output distribution to be specified separately from the dynamics used to realize it. Based on this framework, we introduce FASTER, which trains a small network for each source and objective to perform inexpensive editing, while pretrained and reward models provide feedback on candidate outputs. By reusing each candidate and its feedback across multiple small-network updates, FASTER reduces repeated sampling and supervision queries without placing the pretrained generative backbone inside the inner optimization loop. On SD3, FASTER leads all four target metrics and several validation metrics among the evaluated methods. Compared with the evaluated baseline that optimizes controls along pretrained generation trajectories, FASTER achieves editing-time speedups of up to \({6.91\times}\) on Stable Diffusion 3 and \({24.14\times}\) on Stable Diffusion 1.5.

==> appendices/endpoint.tex <==
\section{Endpoint Realization and Its Scope}
\label{app:theory}
\begin{proposition}[Endpoint realization]
\label{prop:endpoint}
Suppose $\bar\pi_{\vct{s}}$ is positive, has finite $\KL(\bar\pi_{\vct{s}}\Vert q_\tau)$, and its tilted path law
\begin{equation}
 \frac{dP_{\vct{s}}^\star}{dQ_\tau}
 =\frac{\bar\pi_{\vct{s}}(\vct{z}_1)}{q_\tau(\vct{z}_1)}
 \label{eq:optimal-path}
\end{equation}
is realizable by an admissible control. Under the Girsanov and integrability conditions in Appendix~\ref{app:theory},
\begin{equation}
 J_{\vct{s}}(\vct{b})=\KL(P_{\vct{s}}^{\vct{b}}\Vert P_{\vct{s}}^\star).
 \label{eq:kl-identity}
\end{equation}
The unrestricted optimum therefore satisfies $\vct{s}+\vct{z}_1\sim\pi_{\vct{s}}$.
\end{proposition}

\subsection{Assumptions and proof of Proposition~\ref{prop:endpoint}}
Work on continuous residual paths starting at zero. Assume that $\bar\pi_{\vct{s}}$ is positive and normalized, with finite $\KL(\bar\pi_{\vct{s}}\Vert q_\tau)$. For each candidate control, assume the Girsanov stochastic exponential is a true martingale, and the relevant energies and logarithmic expectations are finite. Attaining the optimum within a controlled SDE also requires realizability of the tilted law. Smoothness of a target alone does not establish these conditions.

Set $w_{\vct{s}}(\vct{z})=\bar\pi_{\vct{s}}(\vct{z})/q_\tau(\vct{z})$. Its expectation is
\begin{equation}
 \E_{Q_\tau}[w_{\vct{s}}(\vct{z}_1)]
 =\int q_\tau(\vct{z})\frac{\bar\pi_{\vct{s}}(\vct{z})}{q_\tau(\vct{z})}d\vct{z}=1.
\end{equation}
Consequently $dP_{\vct{s}}^\star/dQ_\tau=w_{\vct{s}}(\vct{z}_1)=e^{-g_{\vct{s}}(\vct{z}_1)}$ defines a probability measure. For any measurable endpoint set $A$,
\begin{equation}
 P_{\vct{s}}^\star(\vct{z}_1\in A)
 =\int_Aq_\tau(\vct{z})w_{\vct{s}}(\vct{z})d\vct{z}
 =\int_A\bar\pi_{\vct{s}}(\vct{z})d\vct{z}.
\end{equation}
The tilt depends only on the endpoint, so the conditional path remains the reference bridge. Expanding the path KL gives
\begin{align}
 \KL(P_{\vct{s}}^{\vct{b}}\Vert P_{\vct{s}}^\star)
 &=\E_{P_{\vct{s}}^{\vct{b}}}\left[
 \log\frac{dP_{\vct{s}}^{\vct{b}}}{dQ_\tau}
 -\log\frac{dP_{\vct{s}}^\star}{dQ_\tau}\right]\\
 &=\KL(P_{\vct{s}}^{\vct{b}}\Vert Q_\tau)+\E_{P_{\vct{s}}^{\vct{b}}}g_{\vct{s}}(\vct{z}_1)\\
 &=\E_{P_{\vct{s}}^{\vct{b}}}\left[
 \int_0^1\frac{\norm{\vct{b}(\vct{z}_t,t;\vct{s})}^2}{2\tau^2}dt
 +g_{\vct{s}}(\vct{z}_1)\right].
\end{align}
The last equality uses Girsanov's path-energy identity. KL is minimized at the target path law whenever that law is realizable. Translation by $\vct{s}$ has unit Jacobian, giving output density $\pi_{\vct{s}}$.

We used normalized densities in $g_{\vct{s}}$. With the unnormalized energy
$F_{\vct{s}}=\alpha D(\vct{s},\cdot)-\gamma\log p_{\mathrm{pre}}-\beta r$, implementation may use $g^0_{\vct{s}}=\log q_\tau+F_{\vct{s}}(\vct{s}+\cdot)$. Then $g^0_{\vct{s}}=g_{\vct{s}}-\log\mathcal Z_{\vct{s}}$ and $J^0=\KL(P^{\vct{b}}_{\vct{s}}\Vert P^\star_{\vct{s}})-\log\mathcal Z_{\vct{s}}$; gradients and minimizers are unchanged.

\subsection{The realizing drift}
Assume
\begin{equation}
 h_{\vct{s}}(\vct{z},t)=\E_{Q_\tau}[e^{-g_{\vct{s}}(\vct{z}_1)}\mid\vct{z}_t=\vct{z}]
 \label{eq:app-h}
\end{equation}
is finite, positive and $C^{1,2}$ at interior times, and its logarithmic gradient defines an admissible nonexplosive diffusion. It solves the backward heat equation. It\^o's formula under $Q_\tau$ gives
\begin{equation}
 dh_{\vct{s}}(\vct{z}_t,t)=\tau\nabla h_{\vct{s}}(\vct{z}_t,t)^\top d\vct{w}_t.
\end{equation}
The normalized process is the conditional likelihood-ratio martingale for the endpoint tilt. Girsanov therefore adds drift
\begin{equation}
 \vct{b}^\star(\vct{z},t;\vct{s})=\tau^2\nabla\log h_{\vct{s}}(\vct{z},t).
 \label{eq:app-doob}
\end{equation}
This realizes the desired path measure under the assumptions. A finite neural family need not contain this drift.

\subsection{Reference scale and source dependence}
For a fixed target, $q_\tau e^{-g_{\vct{s}}}=\bar\pi_{\vct{s}}$, so changing $\tau$ does not change the ideal endpoint. It does change the optimal drift, bridge geometry and numerical behavior. The source-distance penalty and conditional prior regularization have distinct roles, as shown by the mutual-information decomposition in Sec.~\ref{app:conditional-information}.


==> appendices/implementation.tex <==
\section{Controller and Numerical Implementation}
\label{app:implementation}

We parameterize the physical drift as
\begin{equation}
 \vct{b}_{\theta}(\vct{z},t;\vct{s})
 =\vct{m}+f_\psi(\vct{z},t,\vct{s}),\qquad\theta=(\vct{m},\psi),
 \label{eq:parameterization}
\end{equation}
where $\vct{m}\in\R^d$ is a trainable translation and $f_\psi$ supplies state- and time-dependent corrections. Initializing both the translation and the final convolution to zero makes the initial drift identically zero, recovering the Brownian reference.


For a latent tensor of shape $C\times H\times W$, the controller concatenates $\vct{z}$, $\vct{s}$ and a broadcast scalar time into $2C+1$ channels. The nonlinear branch consists of three $3\times3$ convolutions with padding one, channel widths $(2C+1,h,h,C)$, and SiLU after the first two layers. The translation contains $CHW$ trainable scalars. Including all biases, the total number of parameters is
\begin{equation}
 N_\theta=CHW+9h^2+27Ch+11h+C.
\end{equation}
For example, $C=4$, $H=W=64$ and $h=16$ give $20{,}596$ parameters including the translation. This is an architecture example, not a claim that every experimental setting uses those dimensions. The translation and final convolution start at zero; other layers use their usual initialization.

Euler--Maruyama uses independent Gaussian increments as stated in Algorithm~\ref{alg:faster}. Endpoint simulation is detached from controller optimization. The prior model remains frozen and is queried outside the SDE steps. Reward-input gradients still pass through the frozen decoder and reward network; freezing weights does not eliminate those derivatives. After fitting, a fresh independent trajectory produces the output, rather than selecting the best training endpoint.

Experiment-specific values for $K,B,M,N,h$, optimizer rates, prior-query noise levels and replay duration should accompany the final result tables. These are not fixed by the continuous-time propositions. The basic algorithm uses the current endpoint batch; a cache spanning earlier refreshes should be reported as a replay variant.


==> appendices/oracles.tex <==
\section{Endpoint Prior and Reward Oracles}
\label{app:oracle}

The ideal theory uses the clean prior. A conservative surrogate replaces its energy $-\log p_{\mathrm{pre}}$ in Eq.~\eqref{eq:target}. An exact clean score, a noisy diffusion score, and an arbitrary guidance vector are not interchangeable. One possible explicit surrogate is as follows. Let $\ell$ be a noise level sampled from a fixed distribution, $a_\ell$ and $\nu_\ell>0$ fixed corruption coefficients, $p_\ell^{\mathrm{pre}}$ the corresponding pretrained noisy density, and $\vct{\epsilon}$ standard Gaussian noise. Define
\begin{equation}
 \mathcal P_{\mathrm{noise}}(\vct{y})=
 \E_{\ell,\vct{\epsilon}}
 [-\log p_\ell^{\mathrm{pre}}(a_\ell\vct{y}+\nu_\ell\vct{\epsilon})].
 \label{eq:app-prior}
\end{equation}
If differentiation and expectation may be exchanged, its gradient is
$-\E_{\ell,\vct{\epsilon}}[a_\ell\nabla\log p_\ell^{\mathrm{pre}}
 (a_\ell\vct{y}+\nu_\ell\vct{\epsilon})]$.
A pretrained score predictor can supply a Monte Carlo estimate by forward evaluation. This avoids differentiating the score network, but targets $\mathcal P_{\mathrm{noise}}$, not necessarily $-\log p_{\mathrm{pre}}$.

The final implementation must specify the noise-level distribution, score conversion, conditioning, model approximation, and gradient scaling. With an inexact or nonconservative vector estimator, the exact-density interpretation requires qualification. EAM discusses the practical difficulty of obtaining endpoint scores \citep{shin2026eam}, but does not make every noisy-score estimator exact.

For image-space rewards, gradients must pass from $R(\mathcal D(\vct{y}))$ back to $\vct{y}$ even though both networks' weights are frozen. Intermediate activation graphs are released after obtaining the detached endpoint gradient. Source latents and fixed text features can be cached. Learned controller features can only be cached across updates if their producing parameters do not change.


==> appendices/solver.tex <==
\section{Adjoint Sampling and Endpoint Regression}
\label{app:solver}
\begin{proposition}[Consistency of endpoint regression]
\label{prop:regression}
Assume exact labels, sufficient regularity and tail decay, and endpoints distributed as $\bar\pi_{\vct{s}}$. Let
$h_{\vct{s}}(\vct{z},t)=\E_{Q_\tau}[e^{-g_{\vct{s}}(\vct{z}_1)}\mid\vct{z}_t=\vct{z}]$.
The unrestricted population minimizer of Eq.~\eqref{eq:ram-loss} is
\begin{equation}
 \vct{b}^\star(\vct{z},t;\vct{s})
 =\tau^2\nabla\log h_{\vct{s}}(\vct{z},t)
 =\E_{P_{\vct{s}}^\star}[\widehat{\vct{b}}_{\vct{s}}(\vct{z}_1)\mid\vct{z}_t=\vct{z}].
 \label{eq:regression-consistency}
\end{equation}
\end{proposition}

\subsection{Reciprocal projection and path KL}
Let $P$ and $Q_\tau$ share the deterministic initial state, with $P\ll Q_\tau$ and finite path KL. Disintegrating over the terminal state gives
\begin{equation}
 \KL(P\Vert Q_\tau)=\KL(P_1\Vert q_\tau)
 +\E_{z\sim P_1}\KL(P(\cdot\mid Z_1=z)\Vert Q_\tau(\cdot\mid Z_1=z)).
\end{equation}
For $\mathcal R_{Q_\tau}(P)$ the second term vanishes and the first is unchanged. Terminal expectations are also unchanged, so the path-space objective $\KL(P\Vert Q_\tau)+\E_P g_s(Z_1)$ cannot increase. Interpreting the projected law as an admissible drift process additionally requires realizability and the usual Girsanov conditions. This is a property of the exact projection, not a monotonicity guarantee for finite neural regression steps.

\subsection{Control scaling and reference bridges}
In the normalized-control convention of Adjoint Sampling \citep{havens2025adjointsampling}, let $\vct{u}=\vct{b}/\tau$. The physical drift is $\tau\vct{u}$ and the energy is $\norm{\vct{u}}^2/2$. For zero reference drift and no running state cost, the lean adjoint is $\widetilde{\vct{a}}_t=\nabla g_{\vct{s}}(\vct{z}_1)$. Its matching residual satisfies
\begin{equation}
 \frac12\norm{\vct{u}_\theta+\tau\widetilde{\vct{a}}_t}^2
 =\frac1{2\tau^2}\norm{\vct{b}_\theta+\tau^2\nabla g_{\vct{s}}(\vct{z}_1)}^2.
\end{equation}
This gives Eq.~\eqref{eq:drift-target}; the fixed positive loss scale does not affect its unrestricted minimizer.

Under $Q_\tau$, $\Cov(\vct{z}_t,\vct{z}_1)=\tau^2t\mat I$, $\Var(\vct{z}_t)=\tau^2t\mat I$ and $\Var(\vct{z}_1)=\tau^2\mat I$. Gaussian conditioning gives mean $t\vct{z}_1$ and covariance
$\tau^2t\mat I-(\tau^2t\mat I)(\tau^2\mat I)^{-1}(\tau^2t\mat I)=\tau^2t(1-t)\mat I$, proving Eq.~\eqref{eq:bridge}.

\subsection{Proof of Proposition~\ref{prop:regression}}
Let $k(\vct{v}-\vct{z})$ denote the Gaussian transition density with covariance $\tau^2(1-t)\mat I$. Then
\begin{equation}
 h_{\vct{s}}(\vct{z},t)=\int k(\vct{v}-\vct{z})e^{-g_{\vct{s}}(\vct{v})}d\vct{v}.
\end{equation}
Assume differentiation may pass under the integral and boundary terms vanish. Using $\nabla_{\vct{z}}k=-\nabla_{\vct{v}}k$ and integrating by parts,
\begin{align}
 \nabla_{\vct{z}}h_{\vct{s}}
 &=-\int\nabla_{\vct{v}}k(\vct{v}-\vct{z})e^{-g_{\vct{s}}(\vct{v})}d\vct{v}\\
 &=\int k(\vct{v}-\vct{z})\nabla_{\vct{v}}e^{-g_{\vct{s}}(\vct{v})}d\vct{v}\\
 &=-\int k(\vct{v}-\vct{z})e^{-g_{\vct{s}}(\vct{v})}\nabla g_{\vct{s}}(\vct{v})d\vct{v}.
\end{align}
The conditional endpoint density under $P_{\vct{s}}^\star$ is $k(\vct{v}-\vct{z})e^{-g_{\vct{s}}(\vct{v})}/h_{\vct{s}}(\vct{z},t)$. Dividing by $h_{\vct{s}}$ and multiplying by $\tau^2$ gives Eq.~\eqref{eq:regression-consistency}.

The endpoint tilt leaves reference conditional bridges unchanged; hence sampling an endpoint from $\bar\pi_{\vct{s}}$ and a reference bridge produces the joint marginal of $P_{\vct{s}}^\star$. For a square-integrable label $B$ and conditioning state $X$, write $m(X)=\E[B\mid X]$. Expanding the square yields
\begin{equation}
 \E[\norm{a(X)-B}^2\mid X]
 =\norm{a(X)-m(X)}^2+\E[\norm{B-m(X)}^2\mid X],
\end{equation}
since the cross term has zero conditional mean. The optimal predictor is therefore the conditional mean derived above.

\subsection{Finite updates and replay}
For a general frozen endpoint law $\rho_k$, the regression mean is taken under $\rho_k(\vct{z}_1)Q_\tau(d\vct{z}_t\mid\vct{z}_1)$. The proof establishes the target fixed point, not a one-step exact solution or global convergence. Resampling bridges supplies stochastic gradients of the frozen empirical regression objective, not new independent terminal information. Retaining older batches further changes the sampling distribution.


==> sections/algorithm.tex <==
\begin{algorithm}[t]
\caption{FASTER: source-conditioned endpoint refinement}
\label{alg:faster}
\begin{algorithmic}[1]
\Require Source $\vct{s}$; prior-score estimator $\widehat{\vct{s}}_{\mathrm{pre}}$; reward $r$; preservation cost $D$.
\Require Weights $\alpha,\beta,\gamma$; noise scale $\tau$; refreshes $K$; updates $M$; SDE steps $N$.
\State Initialize $\theta=(\vct{m},\psi)$ with $\vct{b}_\theta=0$ and buffer $\mathcal B=\emptyset$; set $\Delta t=1/N$.
\For{$k=1,\ldots,K$}
  \State Initialize one residual $\vct{z}_0=0$.
  \For{$n=0,\ldots,N-1$}
    \State Draw $\vct{\xi}_n\sim\Normal(0,\mat I)$ and update:
    \Statex \hspace{\algorithmicindent}$\displaystyle
      \vct{z}_{n+1}\gets\vct{z}_n
      +\Delta t\,\vct{b}_\theta(\vct{z}_n,n\Delta t;\vct{s})
      +\tau\sqrt{\Delta t}\,\vct{\xi}_n.$
  \EndFor
  \State Detach $\vct{z}\gets\vct{z}_N$; set $\vct{y}=\vct{s}+\vct{z}$.
  \State Query $\widehat{\vct{s}}_{\mathrm{pre}}(\vct{y})$, $\nabla r(\vct{y})$, and $\nabla_yD(\vct{s},\vct{y})$.
  \State Form a detached label with Eq.~\eqref{eq:drift-target}; add this endpoint--label pair to $\mathcal B$, evicting old entries beyond capacity.
  \For{$j=1,\ldots,M$}
    \State Draw a minibatch of endpoints and labels from $\mathcal B$.
    \State Sample $t,\vct{\epsilon}$ and construct bridge states using Eq.~\eqref{eq:bridge}.
    \State Update only $\theta$ with the minibatch loss in Eq.~\eqref{eq:ram-loss}.
  \EndFor
\EndFor
\State Independently simulate the fitted SDE from zero for $N$ steps, obtaining $\vct{z}_N$.
\State \Return $\vct{y}=\vct{s}+\vct{z}_N$; decode for image output.
\end{algorithmic}
\end{algorithm}


==> sections/method_control.tex <==
\subsection{Auxiliary Stochastic Control for Editing}
\label{sec:method-control}
To realize $\pi_s$, we specialize the SOC in Sec.~\ref{sec:prelim_soc} to zero reference drift and constant diffusion $\tau>0$:
\begin{equation}
 dZ_t=b_\theta(Z_t,t;s)\,dt+\tau\,dB_t,
 \qquad Z_0=0,\qquad Y_t=s+Z_t.
 \label{eq:faster-sde}
\end{equation}
Here $Z_t$ is the editing residual and $B_t$ is standard Brownian motion. Conditional on a source, $Y_0=s$; across sources, $Y_0\sim\mu$. Thus the auxiliary process transports source data into edited data, while its residual representation starts at zero. Its time parameter is independent of the pretrained model's noise time.

Let $P_s^b$ denote the controlled residual path law and $Q_\tau$ the reference law with $b=0$, whose endpoint density is $q_\tau(z)=\Normal(z;0,\tau^2I)$. Writing $\bar\pi_s(z)=\pi_s(s+z)$, choose
\begin{equation}
 \begin{aligned}
 g_s(z)&=\log q_\tau(z)-\log\bar\pi_s(z),\\
 J_s(b)&=\E_{P_s^b}\!\left[
 \int_0^1\frac{\|b(Z_t,t;s)\|^2}{2\tau^2}\,dt+g_s(Z_1)\right].
 \end{aligned}
 \label{eq:faster-soc}
\end{equation}
The density-ratio correction compensates for the reference endpoint distribution; unknown normalizers only add constants to $g_s$. Under the regularity and realizability conditions in Appendix~\ref{app:theory}, $J_s$ equals the path KL to the law joining $\bar\pi_s$ endpoints with reference bridges. Its unrestricted optimum therefore satisfies $s+Z_1\sim\pi_s$.

We parameterize the drift as $b_\theta(z,t;s)=m+f_\psi(z,t,s)$ with a small convolutional network fitted separately for each source; architecture and initialization are given in Appendix~\ref{app:implementation}. Simulating Eq.~\eqref{eq:faster-sde} calls only this controller. The frozen pretrained generator supplies prior information at candidate endpoints.


==> sections/method_solver.tex <==
\subsection{Endpoint Adjoint Regression}
\label{sec:method-solver}

The terminal cost in Eq.~\eqref{eq:faster-soc} specifies what the controller should achieve, but differentiating through every simulated path would make repeated updates expensive. Adjoint Matching instead learns a stochastic control by regressing it onto a target from the \emph{lean adjoint}~\citep{domingoenrich2025adjoint}. With our zero-drift Brownian reference and no running state cost, this adjoint simplifies to~\citep{havens2025adjointsampling}
\begin{equation}
    \frac{d\widetilde{\vct{a}}_t}{dt}=0,
    \qquad \widetilde{\vct{a}}_1=\nabla g_{\vct{s}}(\vct{z}_1),
    \qquad \widetilde{\vct{a}}_t=\nabla g_{\vct{s}}(\vct{z}_1).
    \label{eq:lean-adjoint}
\end{equation}
Here $\widetilde{\vct{a}}_t$ is the lean adjoint, and $\nabla g_{\vct{s}}(\vct{z}_1)$ differentiates the terminal cost at the residual endpoint $\vct{z}_1$. Because it is constant along the reference path, one endpoint gradient replaces a backward adjoint solve. In Adjoint Matching's normalized-control notation, $\vct{u}_\theta=\vct{b}_\theta/\tau$ is regressed toward $-\tau\widetilde{\vct{a}}_t$; our physical-drift target is therefore $-\tau^2\nabla g_{\vct{s}}(\vct{z}_1)$ (Appendix~\ref{app:solver}). For the quadratic preservation cost, we compute its practical approximation as
\begin{equation}
    \widehat{\vct{b}}_{\vct{s}}(\vct{z}_1)
    =(1-\alpha\tau^2)\vct{z}_1
    +\tau^2\gamma\widehat{\vct{s}}_{\mathrm{pre}}(\vct{y})
    +\tau^2\beta\nabla_{\vct{y}}r(\vct{y}),
    \qquad\vct{y}=\vct{s}+\vct{z}_1.
    \label{eq:quadratic-label}
\end{equation}
The first term combines the Gaussian reference correction and the pull toward the source. The other terms use a pretrained-prior score estimate $\widehat{\vct{s}}_{\mathrm{pre}}(\vct{y})$ and the latent reward gradient $\nabla_{\vct{y}}r(\vct{y})$. The estimated score stands in for the clean score $\nabla_{\vct{y}}\log p_{\mathrm{pre}}(\vct{y})$; this approximation does not in general preserve the exact target in Eq.~\eqref{eq:target} (Appendix~\ref{app:oracle}). When reward is defined on images, evaluating its gradient requires differentiating through the frozen decoder and reward model only at the endpoint. We cache and detach the resulting target.

Adjoint Matching's squared-error objective depends on an intermediate state paired with its terminal endpoint. Reciprocal Adjoint Matching, introduced in Adjoint Sampling~\citep{havens2025adjointsampling}, draws the endpoint from the current controller and resamples the intermediate state from the \emph{reference bridge} conditioned on that endpoint. For our Brownian reference, this pair is obtained without replaying a controlled trajectory:
\begin{equation}
    \vct{z}_t=t\vct{z}_1+\tau\sqrt{t(1-t)}\,\vct{\epsilon},
    \qquad t\sim\mathcal U(0,1),\quad
    \vct{\epsilon}\sim\Normal(0,\mat I).
    \label{eq:bridge}
\end{equation}
Here $t$ is uniform in $(0,1)$ and $\vct{\epsilon}$ is independent standard Gaussian noise. Let $\mathcal B$ store endpoints sampled from the current controller together with their evaluated $\widehat{\vct{b}}_{\vct{s}}(\vct{z}_1)$. Combining the adjoint-derived drift target with these bridge samples gives our source-conditioned Reciprocal Adjoint Matching objective~\citep{domingoenrich2025adjoint,havens2025adjointsampling}:
\begin{equation}
    \mathcal L_{\vct{s}}(\theta;\mathcal B)
    =\E_{\vct{z}_1\sim\mathcal B,\,t,\vct{\epsilon}}
    \!\left[\norm{\vct{b}_\theta(\vct{z}_t,t;\vct{s})
                     -\sg[\widehat{\vct{b}}_{\vct{s}}(\vct{z}_1)]}^2\right],
    \label{eq:ram-loss}
\end{equation}
Here $\vct{z}_1\sim\mathcal B$ draws a stored endpoint and its target, and $\sg$ prevents gradients through that target. Relative to the normalized-control matching loss, we omit the constant positive factor $1/(2\tau^2)$; this changes the loss scale but not its minimizer (Appendix~\ref{app:solver}). By resampling $t$ and $\vct{\epsilon}$, several updates reuse each endpoint gradient. If the endpoints follow the exact target law and the clean prior score is available, the population minimizer recovers the drift realizing that law (Proposition~\ref{prop:regression}). Our finite cache and approximate scores do not satisfy those premises exactly. We therefore refresh endpoints after several regression updates and decode a fresh sample from the fitted controller, as in Algorithm~\ref{alg:faster}.

\begin{algorithm}[t]
\caption{FASTER: per-image endpoint refinement}
\label{alg:faster}
\begin{algorithmic}[1]
\Require Source latent $\vct{s}$; reward $r$; weights $\alpha,\beta,\gamma$; scale $\tau$.
\Require Endpoint refreshes $K$; updates $M$ per refresh; SDE steps $N$.
\State Initialize $\vct{b}_\theta=\vct{m}+f_\psi$ to zero.
\For{$k=1,\ldots,K$}
    \State Sample one endpoint $\vct{z}_1$ with Eq.~\eqref{eq:faster-sde} using $N$ SDE steps.
    \State At $\vct{y}=\vct{s}+\vct{z}_1$, compute and cache the detached endpoint target from Eq.~\eqref{eq:quadratic-label}.
    \For{$j=1,\ldots,M$}
        \State Draw a cached endpoint; sample $\vct{z}_t$ by Eq.~\eqref{eq:bridge}.
        \State Update only $\theta$ using Eq.~\eqref{eq:ram-loss}.
    \EndFor
\EndFor
\State Sample a fresh endpoint $\vct{z}_1$ from the fitted controller.
\State \Return $\mathcal D(\vct{s}+\vct{z}_1)$.
\end{algorithmic}
\end{algorithm}

\input{sections/algorithm}


==> sections/method_target.tex <==
\subsection{Source-Conditioned Editing Targets}
\label{sec:method-target}
Let $s,y\in\R^d$ denote source and edited latents. For a source $s$, let $Y\sim T(\cdot\mid s)$ describe the output of an editing procedure. Across sources $S\sim\mu$, its marginal density is
\begin{equation}
 p_T(y)=\int T(y\mid s)\,\mu(ds).
 \label{eq:population}
\end{equation}
Reward alignment suggests the population goal $p_T=p_\beta^\star$, but this alone does not specify source correspondence: $T(\cdot\mid s)=p_\beta^\star$ satisfies it while ignoring the source. To incorporate preservation and allow independent per-image optimization, we use the reward-tilted law as a reference for each conditional:
\begin{equation}
 \min_T\;\E_{S\sim\mu}\!\left[
 \KL(T(\cdot\mid S)\Vert p_\beta^\star)
 +\alpha\E_{Y\sim T(\cdot\mid S)}D(S,Y)\right],\qquad\alpha\geq0.
 \label{eq:conditional-objective}
\end{equation}
Here $D$ measures changes to source content that should be retained; its definition does not require a particular Euclidean distance.
\begin{figure}[t]
    \centering
    \includegraphics[
        width=1.0\linewidth,
        trim=3 8 3 3,
        clip
    ]{figure/motivation.pdf}
    \vspace{-6mm}
    \caption{
    \textbf{From trajectory optimization to endpoint refinement.}
    \textbf{(a)} Trajectory-based reward-guided editing repeatedly updates controls and re-simulates the pretrained generation trajectory.
    \textbf{(b)} FASTER instead specifies a source-conditioned endpoint distribution that balances reward, source fidelity, and prior plausibility, and realizes it using a lightweight transport with endpoint-only prior queries.
    }
    \label{fig:motivation}
\end{figure}
\begin{proposition}[Source-conditioned editing target]
\label{prop:conditional}
Assume finite objective values and
$0<C_s:=\int p_\beta^\star(y)e^{-\alpha D(s,y)}dy<\infty$ for $\mu$-almost every $s$.
Over unrestricted conditional densities, the unique solution of Eq.~\eqref{eq:conditional-objective} is
\begin{equation}
 \pi_s(y)=C_s^{-1}p_\beta^\star(y)e^{-\alpha D(s,y)}.
 \label{eq:conditional-target}
\end{equation}
\end{proposition}
For fixed $s$, the objective is $\KL(T(\cdot\mid s)\Vert\pi_s)-\log C_s$; the full proof is in Appendix~\ref{app:conditional}. This conditional formulation trades reward alignment against preservation. With $\alpha>0$, its output marginal need not equal the original reward tilt; the relation to marginal matching is detailed in the same appendix.

Allowing an independently adjustable prior strength gives the normalizable extension
\begin{equation}
 \pi_s(y)\propto p_{\mathrm{pre}}(y)^\gamma
 \exp[-\alpha D(s,y)+\beta r(y)],
 \label{eq:target}
\end{equation}
with $\gamma=1$ recovering Proposition~\ref{prop:conditional}. The task reward may aggregate multiple weighted objectives, including semantic editing signals evaluated through a separate interface in the implementation.

